Exploring AI-Enabled Cybersecurity Frameworks: Deep-Learning Techniques, GPU Support, and Future Enhancements

Traditional rule-based cybersecurity systems have proven highly effective against known malware threats. However, they face challenges in detecting novel threats. To address this issue, emerging cybersecurity systems are incorporating AI techniques, specifically deep-learning algorithms, to enhance their ability to detect incidents, analyze alerts, and respond to events. While these techniques offer a promising approach to combating dynamic security threats, they often require significant computational resources. Therefore, frameworks that incorporate AI-based cybersecurity mechanisms need to support the use of GPUs to ensure optimal performance. Many cybersecurity framework vendors do not provide sufficiently detailed information about their implementation, making it difficult to assess the techniques employed and their effectiveness. This study aims to overcome this limitation by providing an overview of the most used cybersecurity frameworks that utilize AI techniques, specifically focusing on frameworks that provide comprehensive information about their implementation. Our primary objective is to identify the deep-learning techniques employed by these frameworks and evaluate their support for GPU acceleration. We have identified a total of \emph{two} deep-learning algorithms that are utilized by \emph{three} out of 38 selected cybersecurity frameworks. Our findings aim to assist in selecting open-source cybersecurity frameworks for future research and assessing any discrepancies between deep-learning techniques used in theory and practice.

==> sections/05_Techniques.tex <==


\section{Possible Enhancements to Existing Frameworks}
\label{sec:techniques}

The fact that existing frameworks do not make use of \ac{DL}, as we outline in \Cref{ssec:emplTechniques}, begs the question of whether the research literature provides useful approaches to solving cybersecurity tasks with the help of \ac{DL}. First, we will outline promising examples from recent research before we discuss possible limitations and the viability of their use in current commercially available cybersecurity frameworks. 

% Techniques
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Techniques}
\label{ssec:techniques}

We have selected three approaches from recent literature that present novel approaches to solving problems in the fields of \ac{IDPS}, \ac{EDR}, and \ac{IAM}.

\paragraph{A Novel Convolutional Neural Network Approach With Synthetic Attack Data Generator.}
Detecting and preventing intrusions into computer systems and networks is a popular topic in cybersecurity research. Typical examples for this category include analysis of network traffic or computer system internals. As we have described in \Cref{ssec:emplTechniques}, existing frameworks are already using \acp{LSTM} to detect anomalous network traffic. Using \acp{CNN} for intrusion detection has been proposed by various authors~\cite{berman_survey_2019}. Here, we focus on a recent approach presented by \citet{le_imids_2022}, which promises improved detection of network anomalies.

IMIDS (Intelligent Malware Intrusion Detection System) is a two-phase system that consists of the training and prediction stages. It incorporates several key components, including a network capture block that extracts network flows from raw network packets, a feature extraction block that calculates network flow statistics, and an attack detection model based on a ten-layer \ac{CNN}. The \ac{CNN} architecture includes convolutional, max-pooling, and fully connected layers. The model undergoes offline training using labeled network data and is updated periodically with novel attack data. The IMIDS model achieves high detection accuracy, with 96.69\% and 95.92\% average accuracy for the UNSW-NB15~\cite{moustafa_unsw-nb15_2015} and CICIDS2017~\cite{sharafaldin_toward_2018} datasets, respectively~\cite{le_imids_2022}.

\paragraph{A Novel Convolutional Neural Network Approach Using Malware Visualization.}
\ac{EDR} techniques are aimed at improving endpoint security, i.e., for example, detecting and counteracting malware. From our review of existing cybersecurity solutions, it is clear that existing frameworks are currently not employing deep-learning techniques, but rather make use of \ac{ML}. Morpheus, e.g., uses Random Forests to protect endpoints from malware (see \Cref{ssec:frameworkdescriptions}).
In 2021, \citet{pinhero_malware_2021} presented an approach to classifying malware using \acp{CNN} after converting malware to images.

The study presented a comprehensive analysis of images derived from different-sized executables to identify malware accurately. Various fine-tuned \acp{CNN} were evaluated, with the best results achieved using colored visual images of size 256 x 256. Markov images, representing executables as probabilities of byte pairs, outperformed colored and grayscale images when used for training the classifier. Further improvements were explored by presenting diverse image configurations to CNN architectures. Gabor images, obtained by applying Gabor filters and representing textures, demonstrated high accuracies and F-measures. Entropy images, generated by segmenting executables into blocks and computing block entropy, showed similarities among malware variants within specific families. The study identified the most effective \ac{CNN} model architectures and proposed future extensions, including experimenting with a larger dataset, and investigating multimodal image classification using various image representations~\cite{pinhero_malware_2021}. 

This approach can provide cybersecurity frameworks with an improved capability of detecting malware on a system. 

\paragraph{A Novel Deep Neural Network Approach.}
\ac{IAM} is primarily concerned with protecting data integrity and confidentiality by regulating access to data sources. Detecting malicious actors in a network has many parallels to detecting malicious profiles in social networks, and we can therefore draw on approaches developed to combat them.
In 2021, \citet{xu_deep_2021} presented an approach, called DEC (Deep Entity Classification), to detect abusive accounts in online social networks. Their goal was to identify and remediate abusive accounts in a scalable and precise way, which is also important for cybersecurity frameworks. 

The authors propose a deep neural network model that is trained in two stages. The first stage involves training the deep neural network on a large volume of low-precision data to learn embeddings of raw features. The approximate label data, representing sub-types of abusive accounts, is used to train this multi-task neural network. The outputs of the last hidden layer serve as the learned low-dimensional embeddings. The second stage applies transfer learning, utilizing the embeddings from the first stage, along with high-precision human-labeled data, to train a Gradient-Boosted Decision Trees (GBDT) model for classifying abusive accounts. The GBDT model produces the final classification scores. The model significantly outperforms prior techniques in their evaluation~\cite{xu_deep_2021}.


\paragraph{Other Notable Research Work.}
ParSecureML is a GPU-based cybersecurity framework designed to optimize the performance of secure machine-learning algorithms based on two-party computation. It introduces novel features such as profiling-guided adaptive GPU utilization, fine-grained CPU-GPU cooperation, and compressed transmission for inter-node communication. With an average speedup of 3,380\% compared to its predecessor SecureML, ParSecureML enables efficient and secure data processing in machine learning workflows, without sacrificing performance~\cite{chen_parsecureml_2020}.


% Usability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Operational Viability}
\label{ssec:viability}

While the methods outlined have promising potential to improve the efficacy of existing cybersecurity frameworks, it is crucial to demonstrate their practical viability through various metrics. 
To effectively integrate a new theoretical approach into a cybersecurity framework, the theoretical approach must first be evaluated against various statistical metrics, including F-score, precision, and recall. After proving its theoretical merit, it is equally important to acknowledge the significance of other metrics to ensure that theoretical approaches are viable in a practical setting.
These metrics can vary depending on the specific use case of the framework and may include factors such as inference speed, preprocessing requirements, and hardware specifications for optimal performance, alongside the challenges discussed in \Cref{ssec:dlchallenges}. 
Researchers should therefore consider addressing these issues in their work to ensure that their approach can be successfully integrated into a cybersecurity framework and used in a practical scenario.

The following paragraphs offer a discussion with a series of questions that must be addressed prior to integrating the presented techniques.


\paragraph{What data is required for training?} 
IMIDS used labeled network data for model training. Since quality network data is especially hard to obtain, as we touched on in \Cref{ssec:dlchallenges}, they found a way to supplement their training through a custom attack data generator~\cite{le_imids_2022}. If this generator can prove to be effective in practical trials to help reduce the need for human-labeled data, it boosts the feasibility of integrating deep-learning-based network intrusion detectors.

Quality malware datasets are easier to obtain, thus, data is not the biggest concern for the approach presented by \citeauthor{pinhero_malware_2021}.

The matter of DEC on the other hand is not quite as simple. Facebook's data, which was utilized in the study, was partially annotated by hand~\cite{xu_deep_2021}, making any transition to the use of network user data or organizational accounts less clear-cut. While collecting this type of data may be practical for those seeking to monitor their entire network using a cybersecurity framework, other organizations may opt to ignore DEC altogether due to its reliance on capturing a comprehensive view of the network in order to provide meaningful insights.


\paragraph{What hardware resources are crucial for optimal training performance, and what is the approximate duration of the training process?}
While the methodologies proposed by both \citeauthor{le_imids_2022} and \citeauthor{pinhero_malware_2021} do not explicitly mention the use of GPUs, it is reasonable to assume that leveraging GPUs would significantly enhance training, given that both models employ \acp{CNN}.

As pointed out in the study by \citeauthor{xu_deep_2021}, DEC incurs a considerable computational load, but it can be a valuable tool for reducing overall computational burden by removing abusive accounts. However, this reduction of computational load may not occur in network intrusion or \ac{IAM} settings, and thus may only be suitable for specific products.

\paragraph{Is it feasible for the model to be easily re-trained after deployment, and can users perform this re-training?}
In the study by \citeauthor{le_imids_2022}, IMIDS is frequently retrained with novel attack data~\cite{le_imids_2022}, but none of the other two techniques address the topic of re-training specifically. However, it is unlikely that re-training through a user would be feasible in all cases, primarily due to the high data requirements.

% \paragraph{Is it possible to train the model in a federated manner?}
% None of the existing techniques address the topic of federated learning specifically. 

% \paragraph{Can the technique still be utilized proficiently even if the data used for training is unlabeled?}


\paragraph{Is the approach evaluated on recent state-of-the-art datasets or real-world data?}
The studies conducted by \citeauthor{le_imids_2022} and \citeauthor{pinhero_malware_2021} have employed datasets that are commonly used in the field of cybersecurity~\cite{ferrag_deep_2020}. However, it should be noted that these datasets are a few years old, having been published in 2017 and 2018, respectively. 

The study conducted by \citeauthor{xu_deep_2021} used internal Facebook data without specifying a date. 

\paragraph{What is the model's inference speed?}
While the methods claim fast inference speeds, like the findings presented in the \citeauthor{pinhero_malware_2021} study which reduced malware detection time to 0.87 ms, these claims do not provide a comprehensive evaluation of their efficiency within cybersecurity frameworks. To evaluate efficiency accurately, a performance-accuracy tradeoff comparison between traditional rule-based methods and deep-learning-based methods is required.

Furthermore, preprocessing is an important stage in the detection of malware and should not be overlooked. Certain preprocessing techniques, such as the creation of malware images from binary data, as necessary for the approach proposed by \citeauthor{pinhero_malware_2021}, can considerably increase the detection time as a whole. 

% \paragraph{Is an open-source implementation available?}


% \\
% These questions only provide a brief excerpt from all issues that should be taken into consideration.
